Avoiding Ergodicity Problems in Lattice Discretizations of the Hubbard Model

The Hubbard model arises naturally when electron-electron interactions are added to the tight-binding descriptions of many condensed matter systems. For instance, the two-dimensional Hubbard model on the honeycomb lattice is central to the ab initio description of the electronic structure of carbon nanomaterials, such as graphene. Such low-dimensional Hubbard models are advantageously studied with Markov chain Monte Carlo methods, such as Hybrid Monte Carlo (HMC). HMC is the standard algorithm of the lattice gauge theory community, as it is well suited to theories of dynamical fermions. As HMC performs continuous, global updates of the lattice degrees of freedom, it provides superior scaling with system size relative to local updating methods. A potential drawback of HMC is its susceptibility to ergodicity problems due to so-called exceptional configurations, for which the fermion operator cannot be inverted. Recently, ergodicity problems were found in some formulations of HMC simulations of the Hubbard model. Here, we address this issue directly and clarify under what conditions ergodicity is maintained or violated in HMC simulations of the Hubbard model. We study different lattice formulations of the fermion operator and provide explicit, representative calculations for small systems, often comparing to exact results. We show that a fermion operator can be found which is both computationally convenient and free of ergodicity problems.

==> section/second-response-2.tex <==
%!TEX root =  ../response-2.tex

\section{Reply to the Second Referee}

\begin{quote}
In addition to this, I have the following minor objections(mainly, missing citations and incorrect wording in the text.)
\begin{itemize}
    \item missing citation ([?] instead of number on page 1, the end of the last paragraph.)
    \item missing citation in the beginning of the 1st paragraph on the 2nd page.
    \item page 12, after eq 51 - missing citation.
\end{itemize}
\end{quote}
The missing citations, we believe, are actually footnotes that did not render properly.  We're not sure why this happened as they rendered properly on our \LaTeX\ installations and indeed on the arXiv.  The preview of the resubmission for this response shows all footnotes rendered properly. {\bf Hopefully the editor can help ensure the footnotes appear correctly versions of the manuscript generated internally}.

\begin{quote}\begin{itemize}
    \item page 18, the last paragraph: "$\alpha=1$ case has an in-practice problem caused by isolation..." - I guess, it's $\alpha=0$, in fact?
\end{itemize}\end{quote}
Fixed.

\begin{quote}\begin{itemize}
    \item The 3d paragraph on the 2nd page: I have a feeling that terminology should be corrected. det $M[\phi]$ can be both real-valued and complex valued in BSS, since BSS-QMC algorithm can use discrete fields also coupled with charge. Also, it is first said that det M factorizes in BRS algorithm (it means that exponential formulation is implied), then you again refer to BRS saying that it avoids factorization (thus diagonal formulation is implied). Maybe it's better to fix terminology beforehand and use more strictly defined terms.
\end{itemize}\end{quote}

We agree with the referee that the language here was extremely confusing and mistaken in places.  We have clarified that we always are considering BSS with HMC (noting that in a footnote that the discrete algorithm is ergodic), and ensured that by BSS we always mean exponential while BRS always means diagonal.  Part of the confusion is that with real auxiliary fields the BRS determinant is real and of indefinite sign.  But that doesn't mean it `factorizes' in the same way the exponential (BSS) determinant does, which is due to the conjugate reciprocity uncovered in this work.

\begin{quote}\begin{itemize}
    \item page 34: in ref. [56] the diagonal discretization led to chiral symmetry violations that impacted the CDW order....". In fact, the dependence of SDW order parameter on the step in Euclidean time was studied in [56]. So, SDW should be mentioned here.
\end{itemize}\end{quote}
This is now on page 37 and CDW has been changed to SDW.


\begin{quote}\begin{itemize}
    \item Since the ergodicity issues are the most severe in "exponential" formulation (here they appear not only in "practical", but also in "theoretical" sense, using the authors' terminology), and the authors' suggestion is that the "diagonal" formulation should sometimes be used instead, two these formulation should be directly compared for the lattice larger than 2-site problem. In principle, the figure 17 (4x4 lattice, in Supplementary material) is quite close to such comparison, but it's still not exactly what is needed. In order to really support the claims, one needs direct comparison at the same $\alpha$ for diagonal and exponential formulation, checking also against BSS-QMC results with discrete fields. Now exponential and diagonal formulations are plotted at different $\alpha$, which is confusing, since it well might be that at the same alpha they are actually closer.
    It would be ideal to demonstrate that (at exactly the same parameters of simulation) the results in diagonal formulation are closer to the ones obtained from BSS-QMC due to lack of ergodicity issues despite the fact that additional symmetry violations are imposed in comparison with exponential formulation.
\end{itemize}\end{quote}

We originally chose to focus on $\alpha=0$ so as to reproduce the prior work presented in Ref. [40].  However, we appreciated the desire for an apples-to-apples comparsion and have included an $\alpha=1$ exponential calculation in Fig. 17.
With the very fine integrator in this case we found a difference with BSS at intermediate temporal separations, while that is where the diagonal discretization agrees best.

Note also that we discovered a conventional difference in our code that meant the diagonal discretization was time-reversed compared to the exponential discretization.  Therefore, we time-reversed the diagonal calculations in that figure, bringing them into greater agreement with early-time and late-time BSS and exponential calculations.

\begin{quote}\begin{itemize}
\item Also, it might well be that the observable, chosen to demonstrate it (Euclidean two-point correlator) is not the best one.
I would recommend to use CDW order parameter, e.g. squared charge on sublattice, as it was done in ref. 1807.07025 (see fig. 11 there). At $\alpha=1.0$ it exhibits quite severe effects of ergodicity violations if exponential formulation is used. So, one can compute CDW order parameter using exponential formulation, diagonal formulation and BSS-QMC at sufficiently small $\delta$ (step in Euclidean time), where the results approach continuum limit (it can be controlled using BSS-QMC). If the results from diagonal formulation are closer to BSS-QMC in this regime, the authors' claim is fully justified and the paper can certainly be published in PRB.
In principle, the same study can be done for any other observable, just, I believe, CDW order parameter is the most convenient one.
\end{itemize}
\end{quote}

At the referee's request we have implemented additional correlators, the first time slice of each corresponds to an equal-time order parameter, including a CDW order parameter, as detailed in Appendix D, though not the one discussed in 1807.07025 (but one from Meng et al (2010), Nature), for reasons explained in the text.  We find that the diagonal formulation hits the exact result square on the head while the two ensembles generated from different starting points using the exponential formulation differ from one another and from the exact result.
This bolsters our claim that the diagonal discretization does not suffer from the ergodicity issues of the exponential case, as we believe the referee will now agree.

To keep the presentation simple we re-use ensembles from the two-site case already detailed in Figs 7+8, rather than perform a new BSS-QMC calculation.  However, this answers the same question the referee is after: how well do these other observables do when compared to trustable results (in the BSS case there would still be discretization error, but in the two-site case we can compare against exact continuum diagonalization).
While the exponential case exhibits good symmetry properties, it suffers from ergodicity problems, while the diagonal discretization does not (though the symmetry is broken).  We emphasize that for trustable results one must perform a continuum extrapolation.

At the end of Section III.C demonstrating the ergodicity issue in the two site case, we have added a sentence to point the reader to this new appendix.  We also added one sentence to the conclusion, during the discussion of the SDW order parameter, in the context of compromising on symmetries to reduce ergodicity problems.

\section{Other Modifications}

We corrected a few miscellaneous typos that did not impact meaning.

We found in Ulybyshev PRB 2017 [56] an unsupported passing claim that the complex determinant of their operator (which differs from the diagonal discretization, but still contains a linearized hopping) is free from ergodicity issues, and have included this comment in a footnote in the conclusion:
\begin{quote}
    In Ref.~[56] the authors use a fermion operator not considered here, where transport in time alternates between a linearized hopping operator and interaction through the auxiliary field.  They claim that the simulations are free from ergodicity problems because the determinant is complex, in line with our detailed argument.
\end{quote}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../response-2.tex"
%%% End:

